Marital Sorting on Pre-Marital Preferences for Household Behavior

We examine marital sorting using novel data from a marriage-matching platform that records both a dating-to-marriage pipeline and pre-marital attributes, including preferences for children and for the division of housework and childcare. Unlike census or post-marital surveys, characteristics are collected before matching, and objectively measurable attributes are verified using official documents, providing an ideal setting to study matching and sorting free from post-marital adjustment. Using a multidimensional matching framework across twelve attributes, we find assortative matching along all dimensions. Age is the most salient trait, while preferences for children are second--exceeding education--an economically important margin invisible in standard data. A low-dimensional factor representation shows that fertility preferences constitute a distinct sorting dimension. Exploiting the platform's dating-to-marriage pipeline, we show that sorting on fertility preferences emerges at later serious-relationship stages. A theoretical analysis suggests that the magnitude of sorting along this margin is consistent with the veto model of fertility decisions.

==> figuretable/labor_family_economics_project/summary_statistics_matched_continuous_2015_2024.tex <==

\begin{tabular}[t]{lllrrrrrr}
\toprule
Gender & Year &   & N & mean & median & sd & min & max\\
\midrule
Female & 2015 & Age & 1457 & 35.80 & 35.00 & 6.76 & 22.00 & 73.00\\
 &  & Income (upper limit) & 1448 & 412.91 & 400.00 & 154.70 & 300.00 & 1700.00\\
 &  & Height & 1457 & 158.78 & 158.00 & 5.23 & 142.00 & 188.00\\
 &  & Weight & 1457 & 48.09 & 45.00 & 6.07 & 35.00 & 90.00\\
 &  & Flexibility & 1455 & -0.22 & -0.39 & 0.53 & -1.45 & 1.12\\
 & 2016 & Age & 1968 & 35.77 & 35.00 & 6.23 & 22.00 & 74.00\\
 &  & Income (upper limit) & 1949 & 428.07 & 400.00 & 171.86 & 300.00 & 2100.00\\
 &  & Height & 1968 & 158.64 & 158.00 & 5.16 & 142.00 & 178.00\\
 &  & Weight & 1968 & 47.89 & 45.00 & 5.83 & 35.00 & 75.00\\
 &  & Flexibility & 1964 & -0.20 & -0.36 & 0.51 & -1.45 & 1.12\\
 & 2017 & Age & 2535 & 35.80 & 35.00 & 6.10 & 20.00 & 76.00\\
 &  & Income (upper limit) & 2519 & 443.07 & 400.00 & 198.22 & 300.00 & 2100.00\\
 &  & Height & 2535 & 158.78 & 158.00 & 5.17 & 142.00 & 188.00\\
 &  & Weight & 2535 & 48.03 & 45.00 & 6.19 & 35.00 & 95.00\\
 &  & Flexibility & 2532 & -0.22 & -0.38 & 0.51 & -1.45 & 1.12\\
 & 2018 & Age & 3011 & 35.77 & 35.00 & 6.32 & 21.00 & 75.00\\
 &  & Income (upper limit) & 3005 & 441.53 & 400.00 & 179.51 & 300.00 & 2100.00\\
 &  & Height & 3011 & 158.70 & 158.00 & 5.17 & 142.00 & 178.00\\
 &  & Weight & 3011 & 48.20 & 45.00 & 6.33 & 35.00 & 90.00\\
 &  & Flexibility & 3007 & -0.21 & -0.36 & 0.51 & -1.45 & 1.12\\
 & 2019 & Age & 3763 & 35.72 & 35.00 & 6.42 & 21.00 & 77.00\\
 &  & Income (upper limit) & 3739 & 450.47 & 400.00 & 181.15 & 300.00 & 2100.00\\
 &  & Height & 3763 & 158.70 & 158.00 & 5.15 & 142.00 & 176.00\\
 &  & Weight & 3763 & 48.23 & 45.00 & 6.33 & 35.00 & 95.00\\
 &  & Flexibility & 3758 & -0.21 & -0.36 & 0.50 & -1.45 & 1.12\\
 & 2020 & Age & 4167 & 36.16 & 35.00 & 6.70 & 20.00 & 76.00\\
 &  & Income (upper limit) & 4140 & 467.56 & 400.00 & 196.89 & 300.00 & 2100.00\\
 &  & Height & 4167 & 158.67 & 158.00 & 5.16 & 142.00 & 184.00\\
 &  & Weight & 4167 & 48.55 & 50.00 & 6.40 & 35.00 & 95.00\\
 &  & Flexibility & 4161 & -0.21 & -0.29 & 0.50 & -1.45 & 1.12\\
 & 2021 & Age & 5300 & 36.32 & 35.00 & 7.06 & 20.00 & 74.00\\
 &  & Income (upper limit) & 5260 & 475.27 & 400.00 & 198.39 & 300.00 & 2100.00\\
 &  & Height & 5300 & 158.77 & 158.00 & 5.21 & 142.00 & 182.00\\
 &  & Weight & 5300 & 48.91 & 50.00 & 6.70 & 35.00 & 95.00\\
 &  & Flexibility & 5291 & -0.19 & -0.24 & 0.50 & -1.45 & 1.12\\
 & 2022 & Age & 6115 & 35.90 & 35.00 & 7.00 & 20.00 & 76.00\\
 &  & Income (upper limit) & 6074 & 478.78 & 400.00 & 198.36 & 300.00 & 2100.00\\
 &  & Height & 6115 & 158.72 & 158.00 & 5.24 & 142.00 & 178.00\\
 &  & Weight & 6115 & 48.80 & 50.00 & 6.81 & 35.00 & 95.00\\
 &  & Flexibility & 6105 & -0.20 & -0.24 & 0.50 & -1.45 & 1.12\\
 & 2023 & Age & 6605 & 36.06 & 35.00 & 7.11 & 21.00 & 78.00\\
 &  & Income (upper limit) & 6551 & 489.85 & 400.00 & 208.91 & 300.00 & 2100.00\\
 &  & Height & 6605 & 158.59 & 158.00 & 5.23 & 142.00 & 178.00\\
 &  & Weight & 6605 & 49.09 & 50.00 & 6.97 & 35.00 & 95.00\\
 &  & Flexibility & 6600 & -0.21 & -0.24 & 0.49 & -1.45 & 1.12\\
 & 2024 & Age & 7562 & 36.01 & 35.00 & 7.15 & 23.00 & 75.00\\
 &  & Income (upper limit) & 7511 & 503.62 & 500.00 & 208.45 & 300.00 & 2100.00\\
 &  & Height & 7562 & 158.67 & 158.00 & 5.36 & 142.00 & 180.00\\
 &  & Weight & 7562 & 49.40 & 50.00 & 7.38 & 35.00 & 95.00\\
 &  & Flexibility & 7554 & -0.21 & -0.24 & 0.49 & -1.45 & 1.12\\
Male & 2015 & Age & 1322 & 39.80 & 38.50 & 8.00 & 24.00 & 84.00\\
 &  & Income (upper limit) & 1303 & 746.89 & 600.00 & 336.04 & 300.00 & 2100.00\\
 &  & Height & 1322 & 171.58 & 171.00 & 5.59 & 152.00 & 188.00\\
 &  & Weight & 1322 & 64.81 & 65.00 & 9.01 & 45.00 & 95.00\\
 &  & Flexibility & 1314 & -0.24 & -0.36 & 0.38 & -1.45 & 0.90\\
 & 2016 & Age & 1869 & 39.87 & 39.00 & 7.45 & 23.00 & 87.00\\
 &  & Income (upper limit) & 1851 & 752.67 & 700.00 & 336.91 & 300.00 & 2100.00\\
 &  & Height & 1869 & 171.35 & 170.00 & 5.61 & 152.00 & 188.00\\
 &  & Weight & 1869 & 64.41 & 65.00 & 9.09 & 45.00 & 95.00\\
 &  & Flexibility & 1863 & -0.24 & -0.28 & 0.36 & -1.45 & 0.90\\
 & 2017 & Age & 2472 & 39.97 & 39.00 & 7.20 & 23.00 & 78.00\\
 &  & Income (upper limit) & 2461 & 752.82 & 700.00 & 324.16 & 300.00 & 2100.00\\
 &  & Height & 2472 & 171.60 & 172.00 & 5.62 & 152.00 & 192.00\\
 &  & Weight & 2472 & 64.57 & 65.00 & 9.43 & 45.00 & 95.00\\
 &  & Flexibility & 2466 & -0.24 & -0.24 & 0.34 & -1.45 & 0.90\\
 & 2018 & Age & 2967 & 39.76 & 39.00 & 7.37 & 25.00 & 83.00\\
 &  & Income (upper limit) & 2955 & 758.71 & 700.00 & 319.36 & 300.00 & 2100.00\\
 &  & Height & 2967 & 171.65 & 172.00 & 5.64 & 150.00 & 198.00\\
 &  & Weight & 2967 & 64.93 & 65.00 & 9.51 & 40.00 & 95.00\\
 &  & Flexibility & 2958 & -0.22 & -0.24 & 0.35 & -1.45 & 0.90\\
 & 2019 & Age & 3747 & 39.77 & 39.00 & 7.50 & 21.00 & 81.00\\
 &  & Income (upper limit) & 3741 & 774.61 & 700.00 & 340.54 & 300.00 & 2100.00\\
 &  & Height & 3747 & 171.60 & 172.00 & 5.59 & 146.00 & 194.00\\
 &  & Weight & 3747 & 65.16 & 65.00 & 9.54 & 40.00 & 95.00\\
 &  & Flexibility & 3733 & -0.23 & -0.24 & 0.36 & -1.45 & 0.90\\
 & 2020 & Age & 4149 & 39.86 & 39.00 & 7.63 & 24.00 & 80.00\\
 &  & Income (upper limit) & 4138 & 768.70 & 700.00 & 329.99 & 300.00 & 2100.00\\
 &  & Height & 4149 & 171.76 & 172.00 & 5.84 & 150.00 & 198.00\\
 &  & Weight & 4149 & 65.21 & 65.00 & 9.53 & 40.00 & 95.00\\
 &  & Flexibility & 4139 & -0.21 & -0.24 & 0.35 & -1.45 & 0.90\\
 & 2021 & Age & 5290 & 40.09 & 39.00 & 8.09 & 23.00 & 80.00\\
 &  & Income (upper limit) & 5283 & 775.96 & 700.00 & 349.36 & 300.00 & 2100.00\\
 &  & Height & 5290 & 171.64 & 172.00 & 5.71 & 150.00 & 196.00\\
 &  & Weight & 5290 & 65.39 & 65.00 & 9.59 & 40.00 & 95.00\\
 &  & Flexibility & 5279 & -0.21 & -0.24 & 0.36 & -1.45 & 0.90\\
 & 2022 & Age & 6114 & 39.36 & 38.00 & 7.83 & 23.00 & 89.00\\
 &  & Income (upper limit) & 6099 & 767.95 & 700.00 & 341.42 & 300.00 & 2100.00\\
 &  & Height & 6114 & 171.77 & 172.00 & 5.70 & 150.00 & 198.00\\
 &  & Weight & 6114 & 65.40 & 65.00 & 9.77 & 40.00 & 95.00\\
 &  & Flexibility & 6097 & -0.21 & -0.24 & 0.34 & -1.45 & 0.90\\
 & 2023 & Age & 6602 & 39.39 & 38.00 & 7.95 & 22.00 & 90.00\\
 &  & Income (upper limit) & 6589 & 777.51 & 700.00 & 347.70 & 300.00 & 2100.00\\
 &  & Height & 6602 & 171.60 & 172.00 & 5.70 & 142.00 & 196.00\\
 &  & Weight & 6602 & 65.06 & 65.00 & 9.59 & 40.00 & 95.00\\
 &  & Flexibility & 6589 & -0.21 & -0.24 & 0.34 & -1.45 & 0.90\\
 & 2024 & Age & 7561 & 39.06 & 38.00 & 8.02 & 23.00 & 79.00\\
 &  & Income (upper limit) & 7544 & 782.91 & 700.00 & 347.35 & 300.00 & 2100.00\\
 &  & Height & 7561 & 171.65 & 172.00 & 5.75 & 152.00 & 196.00\\
 &  & Weight & 7561 & 65.19 & 65.00 & 9.88 & 40.00 & 95.00\\
 &  & Flexibility & 7544 & -0.21 & -0.24 & 0.35 & -1.45 & 0.90\\
\bottomrule
\end{tabular}


==> figuretable/labor_family_economics_project/summary_statistics_matched_discrete_2015_2019.tex <==

\begin{tabular}[t]{llrrrrrrrrrrrrrrrrrrrr}
\toprule
  &    & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct.\\
\midrule
Educational level & (1)JuniorHigh & 5 & 0.3 & 7 & 0.4 & 5 & 0.2 & 12 & 0.6 & 3 & 0.1 & 5 & 0.2 & 8 & 0.3 & 13 & 0.4 & 12 & 0.3 & 17 & 0.4\\
 & (2)HighSchool & 138 & 8.7 & 186 & 11.8 & 174 & 8.5 & 228 & 11.1 & 214 & 8.2 & 311 & 12.0 & 250 & 8.2 & 345 & 11.3 & 292 & 7.7 & 376 & 9.9\\
 & (3)Vocational & 485 & 30.7 & 113 & 7.2 & 584 & 28.4 & 175 & 8.5 & 785 & 30.2 & 224 & 8.6 & 836 & 27.5 & 238 & 7.8 & 1015 & 26.7 & 317 & 8.3\\
 & (4)Undergraduate & 733 & 46.5 & 736 & 46.6 & 1069 & 52.1 & 1077 & 52.5 & 1366 & 52.6 & 1409 & 54.2 & 1729 & 56.9 & 1719 & 56.5 & 2180 & 57.4 & 2166 & 57.0\\
 & (5)Graduate & 88 & 5.6 & 273 & 17.3 & 130 & 6.3 & 358 & 17.4 & 159 & 6.1 & 499 & 19.2 & 174 & 5.7 & 624 & 20.5 & 248 & 6.5 & 828 & 21.8\\
 & NA & 129 & 8.2 & 263 & 16.7 & 91 & 4.4 & 203 & 9.9 & 72 & 2.8 & 151 & 5.8 & 43 & 1.4 & 101 & 3.3 & 50 & 1.3 & 93 & 2.4\\
Drink Alcohol level & (1)Never & 245 & 15.5 & 120 & 7.6 & 303 & 14.8 & 164 & 8.0 & 456 & 17.5 & 242 & 9.3 & 475 & 15.6 & 280 & 9.2 & 644 & 17.0 & 356 & 9.4\\
 & (2)SocialOnly & 1159 & 73.4 & 982 & 62.2 & 1583 & 77.1 & 1368 & 66.6 & 1957 & 75.3 & 1749 & 67.3 & 2350 & 77.3 & 2045 & 67.3 & 2849 & 75.0 & 2578 & 67.9\\
 & (3)DrinkRegularly & 53 & 3.4 & 220 & 13.9 & 82 & 4.0 & 337 & 16.4 & 122 & 4.7 & 481 & 18.5 & 186 & 6.1 & 642 & 21.1 & 270 & 7.1 & 813 & 21.4\\
 & NA & 121 & 7.7 & 256 & 16.2 & 85 & 4.1 & 184 & 9.0 & 64 & 2.5 & 127 & 4.9 & 29 & 1.0 & 73 & 2.4 & 34 & 0.9 & 50 & 1.3\\
Smoking level & (1)Never & 1448 & 91.8 & 1164 & 73.8 & 1959 & 95.4 & 1666 & 81.1 & 2520 & 97.0 & 2222 & 85.5 & 2992 & 98.4 & 2707 & 89.0 & 3737 & 98.4 & 3440 & 90.6\\
 & (2)Occasionally & 3 & 0.2 & 69 & 4.4 & 7 & 0.3 & 80 & 3.9 & 11 & 0.4 & 96 & 3.7 & 13 & 0.4 & 115 & 3.8 & 16 & 0.4 & 141 & 3.7\\
 & (3)Regularly & 6 & 0.4 & 89 & 5.6 & 2 & 0.1 & 123 & 6.0 & 4 & 0.2 & 154 & 5.9 & 6 & 0.2 & 145 & 4.8 & 10 & 0.3 & 166 & 4.4\\
 & NA & 121 & 7.7 & 256 & 16.2 & 85 & 4.1 & 184 & 9.0 & 64 & 2.5 & 127 & 4.9 & 29 & 1.0 & 73 & 2.4 & 34 & 0.9 & 50 & 1.3\\
Marital History Dummy & (1)NeverMarried & 1260 & 79.8 & 1040 & 65.9 & 1707 & 83.1 & 1521 & 74.1 & 2250 & 86.6 & 2037 & 78.4 & 2661 & 87.5 & 2478 & 81.5 & 3361 & 88.5 & 3134 & 82.5\\
 & (2)DivorcedOrWidowed & 197 & 12.5 & 282 & 17.9 & 261 & 12.7 & 348 & 17.0 & 285 & 11.0 & 435 & 16.7 & 350 & 11.5 & 489 & 16.1 & 402 & 10.6 & 613 & 16.1\\
 & NA & 121 & 7.7 & 256 & 16.2 & 85 & 4.1 & 184 & 9.0 & 64 & 2.5 & 127 & 4.9 & 29 & 1.0 & 73 & 2.4 & 34 & 0.9 & 50 & 1.3\\
Housework Share Level & (2)DiscussWithPartner & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0\\
 & (3)ShareEqually & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0\\
 & NA & 1578 & 100.0 & 1578 & 100.0 & 2053 & 100.0 & 2053 & 100.0 & 2599 & 100.0 & 2598 & 100.0 & 3040 & 100.0 & 3040 & 100.0 & 3797 & 100.0 & 3796 & 100.0\\
Child Care Share Level & (3)DiscussWithPartner & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0\\
 & (4)ShareEqually & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0\\
 & NA & 1578 & 100.0 & 1578 & 100.0 & 2053 & 100.0 & 2053 & 100.0 & 2599 & 100.0 & 2598 & 100.0 & 3040 & 100.0 & 3040 & 100.0 & 3797 & 100.0 & 3796 & 100.0\\
Desired Child Dummy & (1)DoNotWant & 68 & 4.3 & 57 & 3.6 & 66 & 3.2 & 48 & 2.3 & 80 & 3.1 & 52 & 2.0 & 109 & 3.6 & 70 & 2.3 & 125 & 3.3 & 86 & 2.3\\
 & (2)NoPreference & 199 & 12.6 & 201 & 12.7 & 270 & 13.2 & 296 & 14.4 & 377 & 14.5 & 457 & 17.6 & 463 & 15.2 & 552 & 18.2 & 616 & 16.2 & 728 & 19.2\\
 & (3)Want & 1190 & 75.4 & 1064 & 67.4 & 1632 & 79.5 & 1525 & 74.3 & 2078 & 80.0 & 1963 & 75.5 & 2439 & 80.2 & 2345 & 77.1 & 3022 & 79.6 & 2933 & 77.2\\
 & NA & 121 & 7.7 & 256 & 16.2 & 85 & 4.1 & 184 & 9.0 & 64 & 2.5 & 127 & 4.9 & 29 & 1.0 & 73 & 2.4 & 34 & 0.9 & 50 & 1.3\\
\bottomrule
\end{tabular}


==> figuretable/labor_family_economics_project/summary_statistics_unmatched_continuous_2015_2024.tex <==

\begin{tabular}[t]{lllrrrrrr}
\toprule
Gender & Year &   & N & mean & median & sd & min & max\\
\midrule
Female & 2015 & Age & 8855 & 37.61 & 37.00 & 7.80 & 21.00 & 91.00\\
 &  & Income (upper limit) & 8728 & 432.80 & 400.00 & 188.99 & 300.00 & 2100.00\\
 &  & Height & 8854 & 158.95 & 158.00 & 5.06 & 142.00 & 198.00\\
 &  & Weight & 8851 & 48.22 & 50.00 & 5.88 & 35.00 & 90.00\\
 &  & Flexibility & 8823 & -0.15 & -0.36 & 0.53 & -1.45 & 1.12\\
 & 2016 & Age & 11271 & 37.69 & 36.00 & 7.79 & 21.00 & 79.00\\
 &  & Income (upper limit) & 11170 & 439.61 & 400.00 & 194.15 & 300.00 & 2100.00\\
 &  & Height & 11271 & 158.88 & 158.00 & 5.06 & 142.00 & 182.00\\
 &  & Weight & 11271 & 48.13 & 45.00 & 5.97 & 35.00 & 90.00\\
 &  & Flexibility & 11245 & -0.15 & -0.36 & 0.53 & -1.45 & 1.12\\
 & 2017 & Age & 11078 & 37.35 & 36.00 & 7.75 & 21.00 & 89.00\\
 &  & Income (upper limit) & 10957 & 441.10 & 400.00 & 195.69 & 300.00 & 2100.00\\
 &  & Height & 11078 & 158.89 & 158.00 & 5.08 & 142.00 & 180.00\\
 &  & Weight & 11074 & 48.15 & 45.00 & 5.96 & 35.00 & 95.00\\
 &  & Flexibility & 11058 & -0.18 & -0.36 & 0.52 & -1.45 & 1.12\\
 & 2018 & Age & 11949 & 37.26 & 36.00 & 7.59 & 20.00 & 90.00\\
 &  & Income (upper limit) & 11827 & 455.64 & 400.00 & 197.29 & 300.00 & 2100.00\\
 &  & Height & 11948 & 158.93 & 158.00 & 5.08 & 142.00 & 180.00\\
 &  & Weight & 11947 & 48.29 & 45.00 & 6.14 & 35.00 & 95.00\\
 &  & Flexibility & 11919 & -0.19 & -0.36 & 0.52 & -1.45 & 1.12\\
 & 2019 & Age & 13326 & 37.12 & 36.00 & 7.76 & 20.00 & 80.00\\
 &  & Income (upper limit) & 13199 & 465.45 & 400.00 & 207.74 & 300.00 & 2100.00\\
 &  & Height & 13326 & 158.88 & 158.00 & 5.15 & 142.00 & 182.00\\
 &  & Weight & 13324 & 48.42 & 50.00 & 6.21 & 35.00 & 95.00\\
 &  & Flexibility & 13287 & -0.18 & -0.29 & 0.51 & -1.45 & 1.12\\
 & 2020 & Age & 12986 & 37.44 & 36.00 & 7.90 & 20.00 & 82.00\\
 &  & Income (upper limit) & 12851 & 471.86 & 400.00 & 212.87 & 300.00 & 2100.00\\
 &  & Height & 12986 & 158.82 & 158.00 & 5.16 & 142.00 & 180.00\\
 &  & Weight & 12985 & 48.76 & 50.00 & 6.44 & 35.00 & 95.00\\
 &  & Flexibility & 12952 & -0.17 & -0.24 & 0.51 & -1.45 & 1.12\\
 & 2021 & Age & 14995 & 37.12 & 36.00 & 8.00 & 20.00 & 80.00\\
 &  & Income (upper limit) & 14856 & 475.07 & 400.00 & 212.73 & 300.00 & 2100.00\\
 &  & Height & 14993 & 158.78 & 158.00 & 5.15 & 142.00 & 182.00\\
 &  & Weight & 14993 & 48.82 & 50.00 & 6.67 & 35.00 & 95.00\\
 &  & Flexibility & 14943 & -0.18 & -0.24 & 0.51 & -1.45 & 1.12\\
 & 2022 & Age & 17358 & 36.97 & 36.00 & 7.78 & 20.00 & 78.00\\
 &  & Income (upper limit) & 17166 & 482.38 & 400.00 & 210.84 & 300.00 & 2100.00\\
 &  & Height & 17356 & 158.82 & 158.00 & 5.24 & 142.00 & 184.00\\
 &  & Weight & 17355 & 48.99 & 50.00 & 6.80 & 35.00 & 95.00\\
 &  & Flexibility & 17318 & -0.18 & -0.21 & 0.50 & -1.45 & 1.12\\
 & 2023 & Age & 17816 & 37.31 & 36.00 & 8.17 & 20.00 & 81.00\\
 &  & Income (upper limit) & 17589 & 488.17 & 400.00 & 214.59 & 300.00 & 2100.00\\
 &  & Height & 17811 & 158.88 & 158.00 & 5.29 & 142.00 & 198.00\\
 &  & Weight & 17810 & 49.21 & 50.00 & 6.98 & 35.00 & 95.00\\
 &  & Flexibility & 17759 & -0.18 & -0.21 & 0.50 & -1.45 & 1.12\\
 & 2024 & Age & 19885 & 37.39 & 36.00 & 8.42 & 20.00 & 85.00\\
 &  & Income (upper limit) & 19631 & 499.08 & 500.00 & 220.23 & 300.00 & 2100.00\\
 &  & Height & 19883 & 158.88 & 158.00 & 5.28 & 142.00 & 182.00\\
 &  & Weight & 19881 & 49.42 & 50.00 & 7.13 & 35.00 & 95.00\\
 &  & Flexibility & 19824 & -0.18 & -0.19 & 0.50 & -1.45 & 1.12\\
Male & 2015 & Age & 3011 & 41.55 & 40.00 & 9.31 & 20.00 & 91.00\\
 &  & Income (upper limit) & 2917 & 655.71 & 600.00 & 319.40 & 300.00 & 2100.00\\
 &  & Height & 3010 & 170.95 & 170.00 & 5.77 & 142.00 & 192.00\\
 &  & Weight & 3011 & 64.84 & 65.00 & 9.59 & 35.00 & 95.00\\
 &  & Flexibility & 2978 & -0.22 & -0.36 & 0.35 & -1.45 & 0.90\\
 & 2016 & Age & 4343 & 41.83 & 41.00 & 9.09 & 21.00 & 86.00\\
 &  & Income (upper limit) & 4264 & 676.13 & 600.00 & 333.79 & 300.00 & 2100.00\\
 &  & Height & 4343 & 171.01 & 170.00 & 5.81 & 146.00 & 190.00\\
 &  & Weight & 4343 & 64.90 & 65.00 & 9.55 & 40.00 & 95.00\\
 &  & Flexibility & 4303 & -0.23 & -0.36 & 0.36 & -1.45 & 0.90\\
 & 2017 & Age & 4423 & 42.32 & 41.00 & 9.50 & 20.00 & 86.00\\
 &  & Income (upper limit) & 4372 & 668.57 & 600.00 & 328.97 & 300.00 & 2100.00\\
 &  & Height & 4423 & 171.05 & 170.00 & 5.72 & 144.00 & 192.00\\
 &  & Weight & 4423 & 64.97 & 65.00 & 9.83 & 40.00 & 95.00\\
 &  & Flexibility & 4380 & -0.22 & -0.36 & 0.37 & -1.45 & 0.90\\
 & 2018 & Age & 5584 & 41.93 & 41.00 & 9.03 & 21.00 & 90.00\\
 &  & Income (upper limit) & 5530 & 689.26 & 600.00 & 347.51 & 300.00 & 2100.00\\
 &  & Height & 5584 & 171.32 & 170.00 & 5.88 & 142.00 & 196.00\\
 &  & Weight & 5583 & 65.31 & 65.00 & 9.78 & 35.00 & 95.00\\
 &  & Flexibility & 5534 & -0.22 & -0.36 & 0.36 & -1.45 & 0.90\\
 & 2019 & Age & 6828 & 41.72 & 41.00 & 9.15 & 21.00 & 86.00\\
 &  & Income (upper limit) & 6780 & 693.66 & 600.00 & 352.03 & 300.00 & 2100.00\\
 &  & Height & 6828 & 171.16 & 170.00 & 5.92 & 148.00 & 198.00\\
 &  & Weight & 6828 & 65.90 & 65.00 & 10.21 & 40.00 & 95.00\\
 &  & Flexibility & 6779 & -0.20 & -0.29 & 0.36 & -1.45 & 0.90\\
 & 2020 & Age & 7200 & 42.20 & 41.00 & 9.34 & 20.00 & 89.00\\
 &  & Income (upper limit) & 7169 & 686.25 & 600.00 & 341.82 & 300.00 & 2100.00\\
 &  & Height & 7200 & 171.13 & 170.00 & 5.78 & 146.00 & 192.00\\
 &  & Weight & 7200 & 65.84 & 65.00 & 10.20 & 40.00 & 95.00\\
 &  & Flexibility & 7150 & -0.20 & -0.24 & 0.36 & -1.45 & 0.90\\
 & 2021 & Age & 8320 & 42.01 & 41.00 & 9.39 & 21.00 & 90.00\\
 &  & Income (upper limit) & 8261 & 691.04 & 600.00 & 347.44 & 300.00 & 2100.00\\
 &  & Height & 8320 & 171.19 & 170.00 & 5.88 & 142.00 & 198.00\\
 &  & Weight & 8320 & 66.05 & 65.00 & 10.41 & 35.00 & 95.00\\
 &  & Flexibility & 8282 & -0.21 & -0.24 & 0.35 & -1.45 & 0.90\\
 & 2022 & Age & 10110 & 41.70 & 40.00 & 9.24 & 20.00 & 89.00\\
 &  & Income (upper limit) & 10052 & 692.42 & 600.00 & 346.05 & 300.00 & 2100.00\\
 &  & Height & 10110 & 171.18 & 170.00 & 5.79 & 142.00 & 196.00\\
 &  & Weight & 10110 & 65.97 & 65.00 & 10.36 & 35.00 & 95.00\\
 &  & Flexibility & 10061 & -0.20 & -0.24 & 0.35 & -1.45 & 1.12\\
 & 2023 & Age & 11658 & 41.37 & 40.00 & 9.45 & 20.00 & 93.00\\
 &  & Income (upper limit) & 11595 & 693.48 & 600.00 & 346.76 & 300.00 & 2100.00\\
 &  & Height & 11658 & 171.11 & 170.00 & 5.91 & 142.00 & 194.00\\
 &  & Weight & 11658 & 65.94 & 65.00 & 10.25 & 35.00 & 95.00\\
 &  & Flexibility & 11612 & -0.20 & -0.24 & 0.35 & -1.45 & 0.90\\
 & 2024 & Age & 14307 & 41.45 & 40.00 & 9.68 & 20.00 & 91.00\\
 &  & Income (upper limit) & 14263 & 700.05 & 600.00 & 345.59 & 300.00 & 2100.00\\
 &  & Height & 14306 & 171.17 & 170.00 & 5.84 & 142.00 & 196.00\\
 &  & Weight & 14306 & 66.33 & 65.00 & 10.65 & 35.00 & 95.00\\
 &  & Flexibility & 14237 & -0.19 & -0.21 & 0.35 & -1.45 & 0.90\\
\bottomrule
\end{tabular}


==> figuretable/labor_family_economics_project/summary_statistics_unmatched_discrete_2015_2019.tex <==

\begin{tabular}[t]{llrrrrrrrrrrrrrrrrrrrr}
\toprule
  &    & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct.\\
\midrule
Educational level & (1)JuniorHigh & 47 & 0.5 & 47 & 1.6 & 37 & 0.3 & 53 & 1.2 & 32 & 0.3 & 78 & 1.8 & 40 & 0.3 & 74 & 1.3 & 41 & 0.3 & 84 & 1.2\\
 & (2)HighSchool & 976 & 11.0 & 660 & 21.8 & 1202 & 10.6 & 898 & 20.6 & 1091 & 9.8 & 928 & 20.9 & 1130 & 9.4 & 1085 & 19.3 & 1309 & 9.8 & 1358 & 19.7\\
 & (3)Vocational & 2762 & 31.1 & 358 & 11.8 & 3512 & 31.1 & 543 & 12.5 & 3321 & 29.9 & 564 & 12.7 & 3453 & 28.8 & 704 & 12.5 & 3612 & 27.0 & 875 & 12.7\\
 & (4)Undergraduate & 4491 & 50.5 & 1572 & 51.9 & 5785 & 51.1 & 2295 & 52.6 & 5888 & 52.9 & 2265 & 51.0 & 6487 & 54.1 & 2959 & 52.6 & 7469 & 55.8 & 3586 & 52.0\\
 & (5)Graduate & 518 & 5.8 & 342 & 11.3 & 684 & 6.0 & 513 & 11.8 & 692 & 6.2 & 537 & 12.1 & 777 & 6.5 & 703 & 12.5 & 828 & 6.2 & 823 & 11.9\\
 & NA & 94 & 1.1 & 51 & 1.7 & 90 & 0.8 & 59 & 1.4 & 98 & 0.9 & 71 & 1.6 & 97 & 0.8 & 105 & 1.9 & 121 & 0.9 & 164 & 2.4\\
Drink Alcohol level & (1)Never & 1484 & 16.7 & 399 & 13.2 & 1882 & 16.6 & 540 & 12.4 & 1866 & 16.8 & 551 & 12.4 & 1973 & 16.5 & 755 & 13.4 & 2132 & 15.9 & 881 & 12.8\\
 & (2)SocialOnly & 6907 & 77.7 & 2165 & 71.5 & 8751 & 77.4 & 3091 & 70.9 & 8578 & 77.1 & 3127 & 70.4 & 9092 & 75.9 & 3801 & 67.5 & 9984 & 74.6 & 4469 & 64.9\\
 & (3)DrinkRegularly & 463 & 5.2 & 447 & 14.8 & 637 & 5.6 & 712 & 16.3 & 631 & 5.7 & 744 & 16.7 & 881 & 7.4 & 1027 & 18.2 & 1207 & 9.0 & 1475 & 21.4\\
 & NA & 34 & 0.4 & 19 & 0.6 & 40 & 0.4 & 18 & 0.4 & 47 & 0.4 & 21 & 0.5 & 38 & 0.3 & 47 & 0.8 & 57 & 0.4 & 65 & 0.9\\
Smoking level & (1)Never & 8711 & 98.0 & 2457 & 81.1 & 11136 & 98.5 & 3708 & 85.0 & 10939 & 98.4 & 3710 & 83.5 & 11805 & 98.5 & 4840 & 86.0 & 13169 & 98.4 & 5895 & 85.6\\
 & (2)Occasionally & 78 & 0.9 & 201 & 6.6 & 76 & 0.7 & 264 & 6.1 & 90 & 0.8 & 294 & 6.6 & 89 & 0.7 & 325 & 5.8 & 89 & 0.7 & 382 & 5.5\\
 & (3)Regularly & 65 & 0.7 & 353 & 11.7 & 58 & 0.5 & 371 & 8.5 & 46 & 0.4 & 418 & 9.4 & 52 & 0.4 & 418 & 7.4 & 65 & 0.5 & 547 & 7.9\\
 & NA & 34 & 0.4 & 19 & 0.6 & 40 & 0.4 & 18 & 0.4 & 47 & 0.4 & 21 & 0.5 & 38 & 0.3 & 47 & 0.8 & 57 & 0.4 & 66 & 1.0\\
Marital History Dummy & (1)NeverMarried & 7396 & 83.2 & 2331 & 76.9 & 9559 & 84.5 & 3460 & 79.3 & 9528 & 85.7 & 3398 & 76.5 & 10336 & 86.2 & 4458 & 79.2 & 11507 & 86.0 & 5528 & 80.2\\
 & (2)DivorcedOrWidowed & 1458 & 16.4 & 679 & 22.4 & 1711 & 15.1 & 883 & 20.2 & 1549 & 13.9 & 1024 & 23.0 & 1610 & 13.4 & 1125 & 20.0 & 1817 & 13.6 & 1296 & 18.8\\
 & NA & 34 & 0.4 & 20 & 0.7 & 40 & 0.4 & 18 & 0.4 & 45 & 0.4 & 21 & 0.5 & 38 & 0.3 & 47 & 0.8 & 56 & 0.4 & 66 & 1.0\\
Housework Share Level & (1)LeaveToPartner & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0\\
 & (2)DiscussWithPartner & 0 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 0 & 0.0 & 2 & 0.0 & 1 & 0.0 & 1 & 0.0\\
 & (3)ShareEqually & 0 & 0.0 & 1 & 0.0 & 2 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 4 & 0.1\\
 & (4)DoItMyself & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0\\
 & NA & 8888 & 100.0 & 3027 & 99.9 & 11306 & 100.0 & 4359 & 100.0 & 11119 & 100.0 & 4441 & 100.0 & 11982 & 100.0 & 5627 & 99.9 & 13378 & 100.0 & 6884 & 99.9\\
Child Care Share Level & (1)DoNotWantChildren & 0 & 0.0 & 1 & 0.0 & 2 & 0.0 & 1 & 0.0 & 1 & 0.0 & 0 & 0.0 & 2 & 0.0 & 1 & 0.0 & 0 & 0.0 & 1 & 0.0\\
 & (3)DiscussWithPartner & 0 & 0.0 & 1 & 0.0 & 2 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1 & 0.0 & 0 & 0.0 & 2 & 0.0 & 1 & 0.0 & 1 & 0.0\\
 & (4)ShareEqually & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 4 & 0.1\\
 & NA & 8888 & 100.0 & 3027 & 99.9 & 11306 & 100.0 & 4359 & 100.0 & 11120 & 100.0 & 4442 & 100.0 & 11982 & 100.0 & 5627 & 99.9 & 13378 & 100.0 & 6884 & 99.9\\
Desired Child Dummy & (1)DoNotWant & 690 & 7.8 & 157 & 5.2 & 888 & 7.9 & 204 & 4.7 & 795 & 7.1 & 258 & 5.8 & 783 & 6.5 & 277 & 4.9 & 925 & 6.9 & 289 & 4.2\\
 & (2)NoPreference & 1637 & 18.4 & 607 & 20.0 & 2045 & 18.1 & 891 & 20.4 & 1969 & 17.7 & 988 & 22.2 & 2326 & 19.4 & 1306 & 23.2 & 2702 & 20.2 & 1744 & 25.3\\
 & (3)Want & 6522 & 73.4 & 2245 & 74.1 & 8335 & 73.7 & 3248 & 74.5 & 8308 & 74.7 & 3176 & 71.5 & 8829 & 73.7 & 3997 & 71.0 & 9686 & 72.4 & 4788 & 69.5\\
 & NA & 39 & 0.4 & 21 & 0.7 & 42 & 0.4 & 18 & 0.4 & 50 & 0.4 & 21 & 0.5 & 46 & 0.4 & 50 & 0.9 & 67 & 0.5 & 69 & 1.0\\
\bottomrule
\end{tabular}


==> figuretable/labor_family_economics_project/summary_statistics_unmatched_discrete_2020_2024.tex <==

\begin{tabular}[t]{llrrrrrrrrrrrrrrrrrrrr}
\toprule
  &    & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct.\\
\midrule
Educational level & (1)JuniorHigh & 39 & 0.3 & 103 & 1.4 & 48 & 0.3 & 126 & 1.5 & 50 & 0.3 & 106 & 1.0 & 51 & 0.3 & 120 & 1.0 & 60 & 0.3 & 125 & 0.9\\
 & (2)HighSchool & 1289 & 9.9 & 1524 & 21.0 & 1433 & 9.5 & 1660 & 19.8 & 1669 & 9.6 & 1979 & 19.5 & 1739 & 9.7 & 2179 & 18.6 & 1973 & 9.9 & 2661 & 18.5\\
 & (3)Vocational & 3469 & 26.6 & 936 & 12.9 & 3903 & 25.9 & 1102 & 13.1 & 4274 & 24.5 & 1260 & 12.4 & 4416 & 24.7 & 1444 & 12.3 & 4845 & 24.3 & 1719 & 12.0\\
 & (4)Undergraduate & 7329 & 56.1 & 3649 & 50.4 & 8500 & 56.4 & 4250 & 50.7 & 10091 & 57.9 & 5236 & 51.5 & 10385 & 58.1 & 6079 & 51.9 & 11612 & 58.2 & 7514 & 52.3\\
 & (5)Graduate & 797 & 6.1 & 890 & 12.3 & 1023 & 6.8 & 1070 & 12.8 & 1190 & 6.8 & 1404 & 13.8 & 1131 & 6.3 & 1701 & 14.5 & 1285 & 6.4 & 2105 & 14.6\\
 & NA & 130 & 1.0 & 143 & 2.0 & 172 & 1.1 & 181 & 2.2 & 147 & 0.8 & 185 & 1.8 & 166 & 0.9 & 198 & 1.7 & 194 & 1.0 & 247 & 1.7\\
Drink Alcohol level & (1)Never & 2123 & 16.3 & 940 & 13.0 & 2559 & 17.0 & 1113 & 13.3 & 3135 & 18.0 & 1366 & 13.4 & 3560 & 19.9 & 1711 & 14.6 & 4176 & 20.9 & 2223 & 15.5\\
 & (2)SocialOnly & 9527 & 73.0 & 4719 & 65.1 & 10574 & 70.1 & 5328 & 63.5 & 11983 & 68.8 & 6401 & 62.9 & 11854 & 66.3 & 7213 & 61.5 & 12983 & 65.0 & 8876 & 61.8\\
 & (3)DrinkRegularly & 1331 & 10.2 & 1538 & 21.2 & 1847 & 12.2 & 1872 & 22.3 & 2224 & 12.8 & 2340 & 23.0 & 2392 & 13.4 & 2728 & 23.3 & 2715 & 13.6 & 3200 & 22.3\\
 & NA & 72 & 0.6 & 48 & 0.7 & 99 & 0.7 & 76 & 0.9 & 79 & 0.5 & 63 & 0.6 & 82 & 0.5 & 69 & 0.6 & 95 & 0.5 & 72 & 0.5\\
Smoking level & (1)Never & 12808 & 98.1 & 6230 & 86.0 & 14803 & 98.2 & 7227 & 86.1 & 17135 & 98.4 & 8891 & 87.4 & 17598 & 98.4 & 10292 & 87.8 & 19615 & 98.2 & 12716 & 88.5\\
 & (2)Occasionally & 103 & 0.8 & 396 & 5.5 & 118 & 0.8 & 514 & 6.1 & 123 & 0.7 & 552 & 5.4 & 111 & 0.6 & 614 & 5.2 & 126 & 0.6 & 597 & 4.2\\
 & (3)Regularly & 69 & 0.5 & 571 & 7.9 & 61 & 0.4 & 573 & 6.8 & 91 & 0.5 & 664 & 6.5 & 98 & 0.5 & 746 & 6.4 & 133 & 0.7 & 986 & 6.9\\
 & NA & 73 & 0.6 & 48 & 0.7 & 97 & 0.6 & 75 & 0.9 & 72 & 0.4 & 63 & 0.6 & 81 & 0.5 & 69 & 0.6 & 95 & 0.5 & 72 & 0.5\\
Marital History Dummy & (1)NeverMarried & 11154 & 85.5 & 5823 & 80.4 & 13019 & 86.3 & 6704 & 79.9 & 15125 & 86.8 & 8268 & 81.3 & 15556 & 87.0 & 9686 & 82.6 & 17220 & 86.2 & 11844 & 82.4\\
 & (2)DivorcedOrWidowed & 1830 & 14.0 & 1374 & 19.0 & 1968 & 13.1 & 1612 & 19.2 & 2228 & 12.8 & 1839 & 18.1 & 2255 & 12.6 & 1969 & 16.8 & 2657 & 13.3 & 2456 & 17.1\\
 & NA & 69 & 0.5 & 48 & 0.7 & 92 & 0.6 & 73 & 0.9 & 68 & 0.4 & 63 & 0.6 & 77 & 0.4 & 66 & 0.6 & 92 & 0.5 & 71 & 0.5\\
Housework Share Level & (1)LeaveToPartner & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 2 & 0.0 & 6 & 0.0 & 80 & 0.7 & 17 & 0.1 & 102 & 0.7\\
 & (2)DiscussWithPartner & 1 & 0.0 & 4 & 0.1 & 7 & 0.0 & 5 & 0.1 & 11 & 0.1 & 15 & 0.1 & 2826 & 15.8 & 1594 & 13.6 & 5742 & 28.8 & 3364 & 23.4\\
 & (3)ShareEqually & 2 & 0.0 & 7 & 0.1 & 0 & 0.0 & 6 & 0.1 & 11 & 0.1 & 8 & 0.1 & 6621 & 37.0 & 4900 & 41.8 & 10174 & 50.9 & 8316 & 57.9\\
 & (4)DoItMyself & 2 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 2 & 0.0 & 1 & 0.0 & 1099 & 6.1 & 347 & 3.0 & 1553 & 7.8 & 553 & 3.8\\
 & NA & 13048 & 100.0 & 7234 & 99.8 & 15072 & 100.0 & 8378 & 99.9 & 17397 & 99.9 & 10144 & 99.7 & 7336 & 41.0 & 4800 & 41.0 & 2483 & 12.4 & 2036 & 14.2\\
Child Care Share Level & (1)DoNotWantChildren & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 3 & 0.0 & 1 & 0.0 & 308 & 1.7 & 106 & 0.9 & 953 & 4.8 & 340 & 2.4\\
 & (2)LeaveToPartner & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 5 & 0.0 & 41 & 0.3 & 6 & 0.0 & 43 & 0.3\\
 & (3)DiscussWithPartner & 1 & 0.0 & 4 & 0.1 & 7 & 0.0 & 3 & 0.0 & 10 & 0.1 & 14 & 0.1 & 2818 & 15.8 & 1726 & 14.7 & 5257 & 26.3 & 3445 & 24.0\\
 & (4)ShareEqually & 2 & 0.0 & 7 & 0.1 & 0 & 0.0 & 7 & 0.1 & 9 & 0.1 & 8 & 0.1 & 6492 & 36.3 & 4697 & 40.1 & 9679 & 48.5 & 7846 & 54.6\\
 & (5)DoItMyself & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 2 & 0.0 & 0 & 0.0 & 810 & 4.5 & 316 & 2.7 & 1197 & 6.0 & 532 & 3.7\\
 & NA & 13048 & 100.0 & 7234 & 99.8 & 15072 & 100.0 & 8379 & 99.9 & 17397 & 99.9 & 10147 & 99.8 & 7455 & 41.7 & 4835 & 41.3 & 2877 & 14.4 & 2165 & 15.1\\
Desired Child Dummy & (1)DoNotWant & 968 & 7.4 & 345 & 4.8 & 1090 & 7.2 & 377 & 4.5 & 1253 & 7.2 & 431 & 4.2 & 1459 & 8.2 & 541 & 4.6 & 1887 & 9.4 & 695 & 4.8\\
 & (2)NoPreference & 2844 & 21.8 & 2074 & 28.6 & 3324 & 22.0 & 2436 & 29.0 & 4057 & 23.3 & 3123 & 30.7 & 4445 & 24.8 & 3704 & 31.6 & 5047 & 25.3 & 4659 & 32.4\\
 & (3)Want & 9162 & 70.2 & 4774 & 65.9 & 10559 & 70.0 & 5500 & 65.6 & 12026 & 69.0 & 6551 & 64.4 & 11901 & 66.5 & 7407 & 63.2 & 12923 & 64.7 & 8912 & 62.0\\
 & NA & 79 & 0.6 & 52 & 0.7 & 106 & 0.7 & 76 & 0.9 & 85 & 0.5 & 65 & 0.6 & 83 & 0.5 & 69 & 0.6 & 112 & 0.6 & 105 & 0.7\\
\bottomrule
\end{tabular}


==> figuretable/labor_family_economics_project/summary_statistics_year_matched_discrete_2020_2024.tex <==

\begin{tabular}[t]{llrrrrrrrrrrrrrrrrrrrr}
\toprule
  &    & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct. & N & Pct.\\
\midrule
Educational level & (1)JuniorHigh & 9 & 0.2 & 11 & 0.3 & 12 & 0.2 & 24 & 0.5 & 8 & 0.1 & 24 & 0.4 & 13 & 0.2 & 17 & 0.3 & 11 & 0.1 & 21 & 0.3\\
 & (2)HighSchool & 365 & 8.7 & 446 & 10.6 & 451 & 8.5 & 601 & 11.3 & 503 & 8.2 & 631 & 10.3 & 584 & 8.8 & 717 & 10.8 & 604 & 8.0 & 763 & 10.1\\
 & (3)Vocational & 1090 & 26.0 & 418 & 10.0 & 1351 & 25.4 & 426 & 8.0 & 1489 & 24.3 & 491 & 8.0 & 1557 & 23.5 & 532 & 8.0 & 1709 & 22.6 & 619 & 8.2\\
 & (4)Undergraduate & 2376 & 56.6 & 2296 & 54.7 & 3096 & 58.2 & 3012 & 56.7 & 3686 & 60.1 & 3473 & 56.6 & 3960 & 59.8 & 3666 & 55.4 & 4698 & 62.0 & 4207 & 55.5\\
 & (5)Graduate & 310 & 7.4 & 945 & 22.5 & 372 & 7.0 & 1161 & 21.8 & 408 & 6.6 & 1430 & 23.3 & 468 & 7.1 & 1585 & 23.9 & 504 & 6.7 & 1834 & 24.2\\
 & NA & 45 & 1.1 & 79 & 1.9 & 34 & 0.6 & 92 & 1.7 & 44 & 0.7 & 89 & 1.4 & 39 & 0.6 & 104 & 1.6 & 51 & 0.7 & 133 & 1.8\\
Drink Alcohol level & (1)Never & 713 & 17.0 & 406 & 9.7 & 951 & 17.9 & 545 & 10.3 & 1169 & 19.0 & 658 & 10.7 & 1315 & 19.9 & 758 & 11.4 & 1549 & 20.4 & 912 & 12.0\\
 & (2)SocialOnly & 3079 & 73.4 & 2757 & 65.7 & 3796 & 71.4 & 3422 & 64.4 & 4254 & 69.3 & 3867 & 63.0 & 4415 & 66.7 & 4090 & 61.8 & 4838 & 63.9 & 4661 & 61.5\\
 & (3)DrinkRegularly & 375 & 8.9 & 986 & 23.5 & 553 & 10.4 & 1323 & 24.9 & 692 & 11.3 & 1589 & 25.9 & 875 & 13.2 & 1754 & 26.5 & 1175 & 15.5 & 1988 & 26.2\\
 & NA & 28 & 0.7 & 46 & 1.1 & 16 & 0.3 & 26 & 0.5 & 23 & 0.4 & 24 & 0.4 & 16 & 0.2 & 19 & 0.3 & 15 & 0.2 & 16 & 0.2\\
Smoking level & (1)Never & 4144 & 98.8 & 3836 & 91.4 & 5271 & 99.2 & 4869 & 91.6 & 6084 & 99.1 & 5706 & 93.0 & 6566 & 99.2 & 6139 & 92.7 & 7504 & 99.0 & 7092 & 93.6\\
 & (2)Occasionally & 12 & 0.3 & 157 & 3.7 & 20 & 0.4 & 222 & 4.2 & 16 & 0.3 & 200 & 3.3 & 20 & 0.3 & 212 & 3.2 & 35 & 0.5 & 210 & 2.8\\
 & (3)Regularly & 11 & 0.3 & 156 & 3.7 & 9 & 0.2 & 199 & 3.7 & 15 & 0.2 & 208 & 3.4 & 19 & 0.3 & 251 & 3.8 & 23 & 0.3 & 259 & 3.4\\
 & NA & 28 & 0.7 & 46 & 1.1 & 16 & 0.3 & 26 & 0.5 & 23 & 0.4 & 24 & 0.4 & 16 & 0.2 & 19 & 0.3 & 15 & 0.2 & 16 & 0.2\\
Marital History Dummy & (1)NeverMarried & 3651 & 87.0 & 3455 & 82.4 & 4636 & 87.2 & 4344 & 81.7 & 5439 & 88.6 & 5163 & 84.1 & 5854 & 88.4 & 5580 & 84.3 & 6695 & 88.4 & 6426 & 84.8\\
 & (2)DivorcedOrWidowed & 516 & 12.3 & 694 & 16.5 & 664 & 12.5 & 946 & 17.8 & 676 & 11.0 & 951 & 15.5 & 751 & 11.3 & 1022 & 15.4 & 867 & 11.4 & 1135 & 15.0\\
 & NA & 28 & 0.7 & 46 & 1.1 & 16 & 0.3 & 26 & 0.5 & 23 & 0.4 & 24 & 0.4 & 16 & 0.2 & 19 & 0.3 & 15 & 0.2 & 16 & 0.2\\
Housework Share Level & (1)LeaveToPartner & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 4 & 0.1 & 38 & 0.6 & 2 & 0.0 & 20 & 0.3\\
 & (2)DiscussWithPartner & 1 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 1 & 0.0 & 1 & 0.0 & 1086 & 16.4 & 875 & 13.2 & 2227 & 29.4 & 1596 & 21.1\\
 & (3)ShareEqually & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 2 & 0.0 & 0 & 0.0 & 3 & 0.0 & 2855 & 43.1 & 3368 & 50.9 & 4247 & 56.1 & 5326 & 70.3\\
 & (4)DoItMyself & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 477 & 7.2 & 247 & 3.7 & 693 & 9.1 & 352 & 4.6\\
 & NA & 4194 & 100.0 & 4195 & 100.0 & 5314 & 100.0 & 5314 & 100.0 & 6136 & 100.0 & 6133 & 99.9 & 2199 & 33.2 & 2093 & 31.6 & 408 & 5.4 & 283 & 3.7\\
Child Care Share Level & (1)DoNotWantChildren & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 72 & 1.1 & 39 & 0.6 & 250 & 3.3 & 134 & 1.8\\
 & (2)LeaveToPartner & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 2 & 0.0 & 23 & 0.3 & 0 & 0.0 & 4 & 0.1\\
 & (3)DiscussWithPartner & 1 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 1 & 0.0 & 2 & 0.0 & 1087 & 16.4 & 957 & 14.5 & 2000 & 26.4 & 1702 & 22.5\\
 & (4)ShareEqually & 0 & 0.0 & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 3 & 0.0 & 2888 & 43.6 & 3281 & 49.6 & 4297 & 56.7 & 5107 & 67.4\\
 & (5)DoItMyself & 0 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 1 & 0.0 & 0 & 0.0 & 343 & 5.2 & 222 & 3.4 & 505 & 6.7 & 306 & 4.0\\
 & NA & 4194 & 100.0 & 4195 & 100.0 & 5315 & 100.0 & 5314 & 100.0 & 6136 & 100.0 & 6133 & 99.9 & 2229 & 33.7 & 2099 & 31.7 & 525 & 6.9 & 324 & 4.3\\
Desired Child Dummy & (1)DoNotWant & 180 & 4.3 & 105 & 2.5 & 277 & 5.2 & 151 & 2.8 & 300 & 4.9 & 172 & 2.8 & 383 & 5.8 & 198 & 3.0 & 493 & 6.5 & 256 & 3.4\\
 & (2)NoPreference & 765 & 18.2 & 934 & 22.3 & 1046 & 19.7 & 1242 & 23.4 & 1231 & 20.1 & 1485 & 24.2 & 1428 & 21.6 & 1720 & 26.0 & 1652 & 21.8 & 1950 & 25.7\\
 & (3)Want & 3222 & 76.8 & 3110 & 74.1 & 3977 & 74.8 & 3897 & 73.3 & 4584 & 74.7 & 4457 & 72.6 & 4794 & 72.4 & 4684 & 70.7 & 5417 & 71.5 & 5355 & 70.7\\
 & NA & 28 & 0.7 & 46 & 1.1 & 16 & 0.3 & 26 & 0.5 & 23 & 0.4 & 24 & 0.4 & 16 & 0.2 & 19 & 0.3 & 15 & 0.2 & 16 & 0.2\\
\bottomrule
\end{tabular}

